Oscillons and quasi-breathers in D+1 dimensions

We study oscillons in D+1 space-time dimensions using a spherically symmetric ansatz. From Gaussian initial conditions, these evolve by emitting radiation, approaching ``quasi-breathers'', near-periodic solutions to the equations of motion. Using a truncated mode expansion, we numerically determine these quasi-breather solutions in 2<D<6 and the energy dependence on the oscillation frequency. In particular, this energy has a minimum, which in turn depends on the number of spatial dimensions. We study the time evolution and lifetimes of the resulting quasi-breathers, and show how generic oscillons decay into these before disappearing altogether. We comment on the apparent absence of oscillons for D>5 and the possibility of stable solutions for D<2.

==> newcomm.tex <==
\newcommand{\calH}{{\cal H}}
\renewcommand{\d}{\mbox{d}}
\newcommand{\intvecp}{\int \frac{d^3 p}{(2\pi)^3}\,}
\newcommand{\intp}{\int \frac{d^4 p}{(2\pi)^4}\,}
\newcommand{\intq}{\int \frac{d^4 q}{(2\pi)^4}\,}
\newcommand{\intk}{\int \frac{d^4 k}{(2\pi)^4}\,}
\newcommand{\intx}{\int d^4 x\,}
\newcommand{\inty}{\int d^4 y\,}
\newcommand{\intvecx}{\int d^3 x\,}
%
\newcommand{\tR}{\mbox{}^3\!R}
%
\newcommand{\psl}{p\!\!\!/}
%
\newcommand{\ub}{\bar{u}}
\newcommand{\vb}{\bar{v}}
\newcommand{\vecvr}{\boldsymbol{\vr}}
\newcommand{\vecbt}{\boldsymbol{\bt}}
\newcommand{\vecch}{\boldsymbol{\ch}}
\newcommand{\vecsg}{\boldsymbol{\sg}}
\newcommand{\vecSg}{\boldsymbol{\Sg}}
%\pagestyle{empty}
%
\newcommand{\noq}{|\emptyset\rangle}
\newcommand{\vac}{|0\rangle}
\newcommand{\bvac}{\langle 0|}
\newcommand{\qdot}{\dot{q}}
\newcommand{\Adot}{\dot{A}}
\newcommand{\ad}{a^{\dagger}}
\newcommand{\vecj}{{\bf j}}
\newcommand{\vecv}{{\bf v}}
\newcommand{\vecE}{{\bf E}}
\newcommand{\vecB}{{\bf B}}
\newcommand{\vecA}{{\bf A}}
\newcommand{\vecD}{{\bf D}}
\newcommand{\vecf}{{\bf f}}
\newcommand{\veck}{{\bf k}}
\newcommand{\vecl}{{\bf l}}
\newcommand{\vece}{{\bf e}}
\newcommand{\vecp}{{\bf p}}
\newcommand{\vecq}{{\bf q}}
\newcommand{\vecx}{{\bf x}}       %(vette x)
\newcommand{\vecy}{{\bf y}}
\newcommand{\vecz}{{\bf z}}
\newcommand{\vecr}{{\bf r}}
\newcommand{\vecJ}{{\bf J}}
%%
\newcommand{\ko}{\mbox{}^0 \! k}
\newcommand{\kov}{\mbox{}^0 \! \veck}
\newcommand{\phz}{\ph_0}
%
\newcommand{\Uh}{\hat{U}}
\newcommand{\Hh}{\hat{H}}
\newcommand{\vrh}{\hat{\vr}}
\newcommand{\vrt}{\tilde{\vr}}
\newcommand{\vrth}{\hat{\tilde{\vr}}}
\newcommand{\vrthd}{\hat{\tilde{\vr}}^{\dagger}}
\newcommand{\pith}{\hat{\tilde{\pi}}}
\newcommand{\pih}{\hat{\pi}}
\newcommand{\pithd}{\hat{\tilde{\pi}}^{\dagger}}
%
\newcommand{\un}{1\!\!\! 1}
\newcommand{\lag}{\langle}
\newcommand{\rag}{\rangle}
%
\newcommand{\al}{\alpha}
\newcommand{\bt}{\beta}
\newcommand{\gm}{\gamma}
\newcommand{\dl}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\zt}{\zeta}
\newcommand{\et}{\eta}
%\newcommand{\th}{\theta}
\newcommand{\kp}{\kappa}
\newcommand{\lm}{\lambda}
\newcommand{\rh}{\rho}
\newcommand{\sg}{\sigma}
\newcommand{\ta}{\tau}
\newcommand{\phb}{\bar{\ph}}
\newcommand{\ph}{\phi}
\newcommand{\vr}{\varphi}
\newcommand{\ch}{\chi}
\newcommand{\ps}{\psi}
\newcommand{\om}{\omega}
%
\newcommand{\Om}{\Omega}
\newcommand{\Omd}{\Omega^{\dagger}}
\newcommand{\Gm}{\Gamma}
\newcommand{\Lm}{\Lambda}
\newcommand{\Sg}{\Sigma}
%
\newcommand{\vecal}{\mbox{\boldmath $\al$}}
\newcommand{\vecgm}{\mbox{\boldmath $\gm$}}
\newcommand{\vecep}{\mbox{\boldmath $\ep$}}
%
\newcommand{\empt}{|\emptyset\rangle}
%
%\newcommand{\omb}{\overline{\om}}
\newcommand{\psd}{\psi^{\dagger}}
\newcommand{\omt}{\tilde{\om}}
\newcommand{\Vd}{V^{\dagger}}
\newcommand{\Dsl}{D\!\!\!\!/}
\newcommand{\parsl}{\partial\!\!\!/}
\newcommand{\ssl}{s\!\!\!/}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\Th}{\hat{T}}
\newcommand{\qh}{\hat{q}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\quart}{\frac{1}{4}}
\newcommand{\third}{\frac{1}{3}}
\newcommand{\Tr}{\mbox{Tr}\,}  
\newcommand{\unity}{1\!\! 1}
\newcommand{\HDas}{\stackrel{\leftrightarrow}{H_D}}
\newcommand{\dmuas}{\stackrel{\leftrightarrow}{\partial_{\mu}}}
\newcommand{\Dmuas}{\stackrel{\leftrightarrow}{D_{\mu}}}
\newcommand{\dnuasup}{\stackrel{\leftrightarrow}{\partial^{\nu}}}
\newcommand{\dmu}{\partial_{\mu}}
\newcommand{\dm}{\partial_{m}}
\newcommand{\dn}{\partial_{n}}
\newcommand{\dnot}{\partial_{0}}
\newcommand{\dnu}{\partial_{\nu}}
\newcommand{\dmup}{\partial'_{\mu}}
\newcommand{\phd}{\ph^{\dagger}}
\newcommand{\Umux}{U_{\mu x}}
%
%\newcommand{\psb}{\overline{\psi}}
\newcommand{\psb}{\bar{\psi}}
\newcommand{\xib}{\bar{\xi}}
\newcommand{\dlb}{\bar{\dl}}
%\newcommand{\etb}{\overline{\eta}}
\newcommand{\etb}{\bar{\eta}}
\newcommand{\Umx}{U_{\mu}(x)}
\newcommand{\Umdx}{U_{\mu}^{\dagger}(x)}
\newcommand{\Umdxm}{U_{\mu}^{\dagger}(x-a_{\mu}}
\newcommand{\Umdxp}{U_{\mu}^{\dagger}(x+a_{\mu}}
\newcommand{\cb}{\overline{\chi}}
%
\newcommand{\rr}[1]{$^{#1}$}
\newcommand{\eela}[1]{\label{#1}\end{equation}}
\newcommand{\eeala}[1]{\label{#1}\end{eqnarray}}
%
\newcommand{\ra}{\rightarrow}
\newcommand{\aleq}{\mbox{}^{\textstyle <}_{\textstyle\sim}}
\newcommand{\ageq}{\mbox{}^{\textstyle >}_{\textstyle\sim}}
%
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
%
\newcommand{\ahk}{\hat{a}_k}
\newcommand{\ahl}{\hat{a}_l}
\newcommand{\ahdk}{\hat{a}^{\dagger}_k}
\newcommand{\ahdko}{\hat{a}^{\dagger}_{k_1}}
\newcommand{\ahdkp}{\hat{a}^{\dagger}_{k_p}}
\newcommand{\ahdl}{\hat{a}^{\dagger}_l}
\newcommand{\ahlo}{\hat{a}_{l_1}}
\newcommand{\ahlq}{\hat{a}_{l_q}}
\newcommand{\ah}{\hat{a}}
\newcommand{\ahd}{\hat{a}^{\dagger}}
\newcommand{\apko}{a^+_{k_1}}
\newcommand{\apkp}{a^+_{k_p}}
\newcommand{\apl}{a^+_l}
\newcommand{\alo}{a_{l_1}}
\newcommand{\alq}{a_{l_q}}
\newcommand{\Ah}{\hat{A}}
%
\newcommand{\psh}{\hat{\ps}}
\newcommand{\psbh}{\hat{\psb}}
%
\newcommand{\eplus}{\mbox{$\left( \begin{array}{c} 1 \\ 0 \end{array} \right)$}}
\newcommand{\eminus}{\mbox{$\left( \begin{array}{c} 0 \\ 1 \end{array} \right)$}}
\newcommand{\sigp}{\mbox{$\left( \begin{array}{cc} 0 & 1 \\ 0 & 0 \end{array} 
\right)$}}
\newcommand{\sigm}{\mbox{$\left( \begin{array}{cc} 0 & 0 \\ 1 & 0 \end{array} 
\right)$}}
\newcommand{\delsym}{\delta^{k_1 \cdots k_p}_{l_1 \cdots l_q}}
%
\newcommand{\barx}{\bar{x}}
\newcommand{\hnu}{\hat{\nu}}
\newcommand{\amu}{a_{\mu}}
\newcommand{\anu}{a_{\nu}}
\newcommand{\Umuxd}{\Umux^{\dagger}}
%
\newcommand{\dcp}{\delta_{\rm cp}}

